Enhancing Security in Third-Party Library Reuse -- Comprehensive Detection of 1-day Vulnerability through Code Patch Analysis

Nowadays, software development progresses rapidly to incorporate new features. To facilitate such growth and provide convenience for developers when creating and updating software, reusing open-source software (i.e., thirdparty library reuses) has become one of the most effective and efficient methods. Unfortunately, the practice of reusing third-party libraries (TPLs) can also introduce vulnerabilities (known as 1-day vulnerabilities) because of the low maintenance of TPLs, resulting in many vulnerable versions remaining in use. If the software incorporating these TPLs fails to detect the introduced vulnerabilities and leads to delayed updates, it will exacerbate the security risks. However, the complicated code dependencies and flexibility of TPL reuses make the detection of 1-day vulnerability a challenging task. To support developers in securely reusing TPLs during software development, we design and implement VULTURE, an effective and efficient detection tool, aiming at identifying 1-day vulnerabilities that arise from the reuse of vulnerable TPLs. It first executes a database creation method, TPLFILTER, which leverages the Large Language Model (LLM) to automatically build a unique database for the targeted platform. Instead of relying on code-level similarity comparison, VULTURE employs hashing-based comparison to explore the dependencies among the collected TPLs and identify the similarities between the TPLs and the target projects. Recognizing that developers have the flexibility to reuse TPLs exactly or in a custom manner, VULTURE separately conducts version-based comparison and chunk-based analysis to capture fine-grained semantic features at the function levels. We applied VULTURE to 10 real-world projects to assess its effectiveness and efficiency in detecting 1-day vulnerabilities. VULTURE successfully identified 175 vulnerabilities from 178 reused TPLs.

==> Table/ResultAll.tex <==
\begin{table*}[htbp]
\centering
\caption{TPL reuse identification result}
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
  \toprule
  \multirow{2}{*}{\textbf{Target Program}} & \multirow{2}{*}{\textbf{Stars}} & \multirow{2}{*}{\textbf{Lines}} & \multicolumn{3}{c|}{\textbf{Vulture+DB$_{iot}$}} & \multicolumn{3}{c|}{\textbf{Vulture+DB$_{kwd}$}} & \multicolumn{3}{c|}{\textbf{Centris+DB$_{centris}$}} & \multicolumn{3}{c|}{\textbf{Centris+DB$_{iot}$}} & \multicolumn{3}{c}{\textbf{Centris+DB$_{kwd}$}} \\ \cline{4-18} 
  & & & \textbf{TP} & \textbf{FP} & \textbf{P} & \textbf{TP} & \textbf{FP} & \textbf{P} & \textbf{TP} & \textbf{FP} & \textbf{P} & \textbf{TP} & \textbf{FP} & \textbf{P} & \textbf{TP} & \textbf{FP} & \textbf{P} \\ \hline
  AliOS-Things & 4.5K & 4,619K & 30 & 21 & 0.59 & 20 & 41 & 0.33 & 15 & 7 & 0.68 & 36 & 45 & 0.44 & 21 & 57 & 0.27 \\ \hline
  LiteOS & 4.8K & 1,174K & 9 & 11 & 0.45 & 4 & 15 & 0.21 & 6 & 9 & 0.40 & 9 & 17 & 0.35 & 4 & 19 & 0.17 \\ \hline
  Tasmota & 21.4K & 1,587K & 52 & 19 & 0.73 & 39 & 24 & 0.62 & 17 & 11 & 0.61 & 55 & 38 & 0.59 & 41 & 44 & 0.48 \\ \hline
  TizenRT & 0.5K & 2,156K & 31 & 16 & 0.66 & 20 & 31 & 0.39 & 22 & 9 & 0.71 & 37 & 35 & 0.51 & 22 & 46 & 0.32 \\ \hline
  kamailio & 2.1K & 1,164k & 2 & 5 & 0.29 & 2 & 8 & 0.20 & 1 & 2 & 0.33 & 2 & 7 & 0.22 & 2 & 9 & 0.18 \\ \hline
  mbed-os & 4.6K & 8,635K & 10 & 8 & 0.56 & 10 & 18 & 0.36 & 3 & 4 & 0.43 & 10 & 12 & 0.45 & 11 & 24 & 0.31 \\ \hline
  openthread & 3.4K & 451K & 2 & 2 & 0.50 & 1 & 3 & 0.25 & 2 & 0 & 1.00 & 2 & 3 & 0.40 & 1 & 6 & 0.14 \\ \hline
  Sming & 1.4K & 32,326K & 17 & 16 & 0.52 & 3 & 0 & 1.00 & 3 & 2 & 0.60 & 18 & 30 & 0.38 & 5 & 5 & 0.50 \\ \hline
  TDengine & 22.8K & 774K & 3 & 0 & 1.00 & 2 & 2 & 0.50 & 1 & 2 & 0.33 & 3 & 1 & 0.75 & 4 & 5 & 0.44 \\ \hline
  zephyr & 9.7K & 2,180K & 2 & 1 & 0.67 & 1 & 4 & 0.20 & 1 & 0 & 1.00 & 2 & 1 & 0.67 & 1 & 7 & 0.13 \\ \hline
  \textbf{Total} & - & - & \underline{\textbf{158}} & \textbf{99} & \underline{\textbf{0.61}} & \textbf{102} & \textbf{146} & \textbf{0.41} & \textbf{71} & \textbf{46} & \textbf{0.60} & \textbf{174} & \textbf{189} & \textbf{0.47} & \textbf{112} & \underline{\textbf{222}} & \textbf{0.33} \\
  \bottomrule
\end{tabular}
\label{tab:result_all}

\end{table*}

==> Table/cve_patch_align_commit_time.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[t]
\centering
\caption{The Correlation between Number of Candidate Commits and Time Cost}
\label{tab:result_all}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{CVE-ID}                       & \textbf{Num}     & \textbf{VCMatch}        & \textbf{VFCFinder}             & \textbf{\sysname}               \\ \hline
CVE-2011-1764  &  30   &   &  77.03   &  36.73  \\ \hline
CVE-2016-1897  &  42   &   &  49.18   &  19.96  \\ \hline
CVE-2019-10899 &  48   &   &  64.23   &  43.26  \\ \hline
CVE-2016-6306  &  221  &   &  261.85  &  27.45  \\ \hline
CVE-2019-9183  &  294  &   &  485.52  &  45.77  \\ \hline
CVE-2021-28135 &  387  &   &  445.20  &  30.95  \\ \hline
CVE-2022-23094 &  934  &   &  1405.56 &  318.68 \\ \hline
CVE-2007-6441  &  1407 &   &  2225.50 &  107.36 \\ \hline
CVE-2012-5360  &  3831 &   &  4355.09 &  915.87 \\ \hline
\end{tabular}
\end{table}

==> Table/motivation1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[t]
\centering
\caption{Example of zlib Maintenance and Reuse}
\begin{tabularx}{\linewidth}{c|c|c}
\toprule[1.5pt]
\textbf{Project} & \textbf{Time} & \textbf{Action} \\ 
\midrule
\underline{zlib} & 1995-May & Start to maintain at: zlib.net \\ 
Linux & 2005-May & Reused zlib at: \textit{linux/lib/zlib\_deflate} \\ 
TrinityCore & 2010-Aug & Reused zlib at: \textit{dep/zlib} \\ 
\underline{zlib} & 2011-Sep & Mirrored to: github.com/madler/zlib \\
TizenRT & 2018-May & Reused zlib at: \textit{external/grpc/extlib/zlib} \\
\bottomrule[1.5pt]
\end{tabularx}
\label{tab:motivation_example1}
\end{table}

==> Table/related.tex <==
\begin{table*}[htbp]
\centering
\caption{Summary of the Comparison Between \sysname and Related Works}
\label{table:relatedwork}
% \begin{tabularx}{\textwidth}{ccccc | ccccc | cccc}
% \toprule[1.5pt]
% \textbf{Type} & \textbf{Scheme}                                                  & \textbf{C1} & \textbf{C2} & \textbf{C3} & \textbf{Type} & \textbf{Scheme}                                                                       & \textbf{C4} & \textbf{C5} & \textbf{C6} & \textbf{Type} & \textbf{Scheme} & \textbf{C7} & \textbf{C8} \\ \hline
% Token Sim.            & \begin{tabular}[c]{@{}c@{}}SourceerCC\cite{SourcererCC}\\ CCAligner\cite{CCAligner}\end{tabular}   &      \ding{55}       &     \ding{55}        &     \ding{55}        & Retrieval            & \begin{tabular}[c]{@{}c@{}}CVEFixes\cite{cvefixes}\\ V1SCAN\cite{v1scan}\\ Tracer\cite{tracer}\end{tabular}                      &     \ding{55}        &      \ding{51}        &      \ding{55}        & Code Sim.            &       \begin{tabular}[c]{@{}c@{}}ReDeBug\cite{redebug}\\ VUDDY\cite{vuddy}\end{tabular}         &       \ding{55}      &      \ding{55}       \\
% \begin{tabular}[c]{@{}c@{}}Function Sim. \&\\ Pre-Dep. Opt.\end{tabular}           & \begin{tabular}[c]{@{}c@{}}Centris\cite{Centris}\\ OSSFP\cite{OSSFP}\\ TPLite\cite{TPLite}\end{tabular} &       \ding{51}      &         \ding{51}    &      \ding{55}       & Ranking            & \begin{tabular}[c]{@{}c@{}}PatchScout\cite{patchscout}\\ VCMatch\cite{vcmatch}\\ PatchMatch\cite{patchmatch}\\ VFCFinder\cite{vfcfinder}\end{tabular} &      \ding{51}       &     \ding{55}        &      \ding{55}       &       \begin{tabular}[c]{@{}c@{}}Core Feature \&\\ Patch Line\end{tabular}      & \begin{tabular}[c]{@{}c@{}}Movery\cite{movery}\\ V1SCAN\cite{v1scan}\end{tabular}          &   \ding{51}          &      \ding{55}       \\
% \begin{tabular}[c]{@{}c@{}}Function Sim. \&\\ Post-Dep. Opt.\end{tabular}        & \sysname                                                          &     \ding{51}        &     \ding{51}       &      \ding{51}       & Logic            & \sysname                                                                               &      \ding{51}       &      \ding{51}       &    \ding{51}         &     \begin{tabular}[c]{@{}c@{}}Core Feature \&\\ Static Analysis\end{tabular}       & \sysname         &       \ding{51}      &     \ding{51}        \\ 
% \bottomrule[1.5pt]
% \end{tabularx}

\begin{tabular}{ccccc | ccccc | cccc}
\toprule[1.5pt]
\multicolumn{5}{c|}{\textbf{TPL Reuse Detection}} & \multicolumn{5}{c|}{\textbf{Security Patch Collection}} & \multicolumn{4}{c}{\textbf{1-day Vulnerability Detection}} \\ \cmidrule(lr){1-5} \cmidrule(lr){6-10} \cmidrule(lr){11-14}
\textbf{Type} & \textbf{Scheme}                                                  & \textbf{C1} & \textbf{C2} & \textbf{C3} & \textbf{Type} & \textbf{Scheme}                                                                       & \textbf{C4} & \textbf{C5} & \textbf{C6} & \textbf{Type} & \textbf{Scheme} & \textbf{C7} & \textbf{C8} \\ \midrule
Token Sim.            & \cite{SourcererCC, CCAligner} &      \ding{55}       &     \ding{55}        &     \ding{55}        & Retrieval            & \cite{cvefixes, v1scan, tracer}                      &     \ding{55}        &      \ding{51}        &      \ding{55}        & Code Sim.            &     \cite{redebug, vuddy}        &       \ding{55}      &      \ding{55}       \\
\begin{tabular}[c]{@{}c@{}}Function Sim. \&\\ Pre-Dep. Opt.\end{tabular}           & \cite{Centris, OSSFP, TPLite} &       \ding{51}      &         \ding{51}    &      \ding{55}       & Ranking            & \cite{patchscout, vcmatch, vfcfinder} &      \ding{51}       &     \ding{55}        &      \ding{55}       &       \begin{tabular}[c]{@{}c@{}}Semantic Analysis \&\\ Coarse-grained \end{tabular}      & \cite{movery, v1scan,mvp}         &   \ding{51}          &      \ding{55}       \\
\begin{tabular}[c]{@{}c@{}}Function Sim. \&\\ Post-Dep. Opt.\end{tabular}        & \sysname                                                          &     \ding{51}        &     \ding{51}       &      \ding{51}       & Mapping            & \sysname                                                                               &      \ding{51}       &      \ding{51}       &    \ding{51}         &     \begin{tabular}[c]{@{}c@{}}Semantic Analysis \&\\ Fine-grained  \end{tabular}       & \sysname         &       \ding{51}      &     \ding{51}        \\ 
\bottomrule[1.5pt]
\end{tabular}

\begin{tabular}{ll}
\multicolumn{2}{l}{In table, ``Sim.", ``Dep.", ``Opt." refer to ``Similarity", ``Dependency", ``Optimization", respectively; ``C" refers to ``Characteristic".}     \\
\textbf{C1:} Whether the solution can detect custom reused TPLs?                & \textbf{C5:} Does the solution avoid the need for manual verification of top-N results?             \\
\textbf{C2:} Whether the solution can deal with nested TPL dependencies?        & \textbf{C6:} Can the solution handle the absence of the patch commit? \\
\textbf{C3:} Whether the solution is maintainable?                              & \textbf{C7:} Can the solution detect TPL vulnerabilities caused by custom reuse?                                                                     \\
\textbf{C4:} Does the solution not rely on patches provided by other platforms? & \textbf{C8:} Can the solution handle complex custom reuses?                                                         
\end{tabular}
\end{table*}


==> Tex/5_implementation.tex <==
As shown in Figure [?], \sysname is composed of three modules: a multifaceted database construction module, a TPL reuse identification module, and a Software flaw detector. Together, these modules form a tool chain that spans from data collection to flaw detection. In total, \sysname consists of approximately 5000 lines of Python code.

\subsection{Security Patch Matching}




\dk{
For CVE database construction, 
}

\subsection{TPL Reuse Identification}
The TPL reuse identification module takes the target program and the component segment of the database as inputs and generates a reuse report for the target program. This module builds on the foundation of CENTRIS [?], comprising around 870 lines of Python code, and includes significant enhancements with over 300 lines of modifications.

\subsection{Software Flaw Detection}
The software flaw detector, which includes 2,692 lines of Python code, is engineered to uncover unpatched flaws within the target program. For file reformatting, we utilized Clang-format, which significantly reduces inaccuracies caused by inconsistent code formatting. Moreover, we employed Ctags [?], for analyzing C/C++ programs. This tool is essential for accurately identifying program elements such as functions and variables. It is well-maintained, lightweight, and accurate. For the LSH algorithm, we selected TLSH due to its established accuracy and scalability. In alignment with CENTRIS, we set the cutoff threshold for similarity cooperation at 30. Finally, for statement operation detection, a combination of well-designed regular expressions and a recursive visit algorithm was implemented, encompassing 38 distinct regular expressions that cover all statement conditions within the Clang Indexing Library.

==> Tex/7_discussion.tex <==
\textbf{Improvement of the database.} The efficiency of \sysname is significantly enhanced by the database we constructed. However, two key challenges remain in the database construction process. \ding{182} The first challenge is to extend \sysname to other platforms. We have tested \sysname on IoT-related programs, future work can adapt \sysname to other platforms by updating the TPLs in the database.
\ding{183} While NVD utilizes CPE to provide detailed information regarding affected versions, a significant challenge arises due to the difference between CPE versioning formats and those employed by individual TPLs on GitHub. This problem arises from the inconsistent version naming practices employed by certain TPLs. Future work in this domain should prioritize the development of robust methods to bridge this gap and ensure accurate CVE-TPL version alignment. 

\textbf{Overcoming similarity-based detection limitations.} Currently, \sysname suffer from the limitations of similarity-based detection. Specifically, significantly altered reused functions might not meet the preset threshold, leading to false negatives. This issue suggests the need for more sophisticated similarity metrics (e.g. function name, function location) or machine learning models that can better capture function semantics beyond syntactic similarities. 

\textbf{Enhancing chunk-based detection} While chunk-based detection provides significant efficiency benefits, it has limitations in pinpointing the exact locations of modifications within reused TPL code. Future work should focus on enhancing \sysname's data-flow analysis capabilities by employing fine-grained code analysis or data-flow tracking mechanisms.
For example, by tracking data-flow of the variables been modified by the chunk, a more comprehensive understanding of vulnerability can be generated to further support 1-day vulnerability detection.
